XACML 3.0 in Answer Set Programming

We present a systematic technique for transforming XACML 3.0 policies in Answer Set Programming (ASP). We show that the resulting logic program has a unique answer set that directly corresponds to our formalisation of the standard semantics of XACML 3.0 from Ramli et. al. We demonstrate how our results make it possible to use off-the-shelf ASP solvers to formally verify properties of access control policies represented in XACML, such as checking the completeness of a set of access control policies and verifying policy properties.

==> introduction.tex <==
%!TEX root = ../main.tex
%\vspace{-1cm}
\section{Introduction}


% make this less concrete (just say that a policy + request -> decision)
XACML (eXtensible Access Control Markup Language)  is an OASIS\footnote{OASIS (Organization for the Advancement of Structured Information Standard) is a non-for-profit,
global consortium that drives the development, convergence, and adoption of e-business standards. Information about OASIS can be found at \url{http://http://www.oasis-open.org/}.} standard that describes both a policy language and an access control decision request/response language. The policy language is used to describe access control requirements (\textit{who can do what when}). The request/response language is used to form a query to ask whether or not a given action should be allowed (\textit{request}), and describes the answer to the query (\textit{response}). The response  returns an answer in one of four values: \textit{permit} (the access is granted), \textit{deny} (the access is denied), \textit{indeterminate} (a decision cannot be made because there is an error during evaluation of some attributes) or \textit{not applicable} (no policy is relevant to the given request). XACML has been under development for some time -- in this paper we consider the latest version 3.0  ratified by OASIS standards organisation on August 10, 2010 \cite{XACML3.0}.

% this is not really important at this point
In XACML, policies are combined together to produce a single decision. XACML 3.0 enhances XACML 2.0's \cite{XACML2.0} existing combination algorithms in the treatment of the indeterminate value. XACML 3.0 distinguishes between the following three types of indeterminate values:
\begin{enumerate}
	\renewcommand{\labelenumi}{\roman{enumi}.}
	\item \emph{Indeterminate permit} (\ip) -- an indeterminate value arising from a policy which could have been evaluated to permit but not deny;
	\item \emph{Indeterminate deny} (\id) -- an indeterminate value arising from a policy which could have been evaluated to deny but not permit;
	\item \emph{Indeterminate deny permit} (\idp) -- an indeterminate value arising from a policy which could have been evaluated as both deny and permit. 
\end{enumerate}

% 1. policies are big big big
% 2. we want to know what they do -- complete? satisfies some required domain-specific property? 
% 3. we need automatised tools to support the process of policy analysis and property verification
The problem with XACML is that its specification is described in natural language (c.f.\ \cite{XACML3.0}) and manual analysis of the overall effect and consequences of a large XACML policy set is a very daunting and time-consuming task. How can a policy developer be certain that the represented policies capture all possible requests? Can they lead to conflicting decisions for some request? Do the policies satisfy all required properties? These are complex problems that cannot be solved easily without some sort of automatised support. 

% 4. our solution is like Ahn et al. in that we use ASP as the vehicle for analysing/verifying properties of policies (it's practical, efficient, declarative, expressive, blabla)
To address this problem we propose a logic-based XACML analysis framework using Answer Set Programming (ASP). With ASP we model an XACML Policy Decision Point (PDP) that loads XACML policies and evaluates XACML requests against these policies. The expressivity of ASP and existence of efficient implementations of the answer set semantics, such as \texttt{clasp}\footnote{\url{http://www.cs.uni-potsdam.de/clasp/}} and  \texttt{DLV}\footnote{\url{http://www.dlvsystem.com/}}, provides the means for declarative specification and verification of properties of XACML policies.

%ASP has become a popular approach to solve combinatorial problems declaratively. There are several efficient implementations of the answer set semantics, such as . 

% 5. but we do better than Ahn et al. in that instead of translating the natural language description directly into ASP, we translate our formalisation of the XACML semantics which provides a common ground for such tasks :P
Our approach is inspired by the work of Ahn \textit{et al.} \cite{Ahn2010,Ahn2010a}.
% the difference should come earlier
There are three main differences between our approach and the work of Ahn \textit{et al.} First, while they consider XACML version 2.0, we address the newer version 3.0. Second, Ahn \emph{et al.} produce a monolithic logic program that can be used for the analysis of XACML policies while we take a more modular approach by first modelling an XACML PDP as a logic program and then using this encoding within a larger program for property analysis. Finally, Ahn \emph{et al.} translate the XACML specification directly to logic programming, so the ambiguities in the natural language specification of XACML are also reflected in their encodings. Due to these reasons, we base our encodings on our formalisation of XACML from \cite{Ramli2011}.

% so how are you inspired, what is new?
We start our work by presenting the formal semantics of XACML that we introduced in \cite{Ramli2011}. Then we define a step-by-step transformation of XACML policies into logic programs. We conjecture that the unique answer set of the transformed logic program directly corresponds to our formal semantics of XACML.

%, we base our work on the formalisation 

%we define a program that corresponds to the PDP and then use it for the verification of properties of XACML policies

%our work promotes the modularity of the transformedour transformation 


%directly translate the XACML policies based on the XACML specification into ASP programs. Jumping the analyst of the XACML true semantics usually leads a mistake like what happens in  \cite{Bruns2008,Ni2009}, including Ahn \textit{et al.} work \footnote{A minor mistake in Anh \textit{et al.} work is found in the translation of permit-overrides and deny-overrides combining algorithms.}.

\smallskip \noindent \textit{Outline.}
We explain the syntax and semantics of XACML 3.0 in Sect.~\ref{s:xacml}. Then we describe the transformation of XACML 3.0 components into a logic program $\mc{P}_{\textrm{XACML}}$ in Sect.~\ref{s:transformation}. We show the relation between XACML 3.0 semantics and the answer sets of  $\mc{P}_{\textrm{XACML}}$ in Sect.~\ref{s:xacml-asp}. Next, in Sect.~\ref{s:analysis}, we show how to verify access control properties, such as checking the completeness of a set of policies. We end the paper with conclusions and future work. 



